Decentralized Task Offloading and Load-Balancing for Mobile Edge Computing in Dense Networks

We study the problem of decentralized task offloading and load-balancing in a dense network with numerous devices and a set of edge servers. Solving this problem optimally is complicated due to the unknown network information and random task sizes. The shared network resources also influence the users' decisions and resource distribution. Our solution combines the mean field multi-agent multi-armed bandit (MAB) game with a load-balancing technique that adjusts the servers' rewards to achieve a target population profile despite the distributed user decision-making. Numerical results demonstrate the efficacy of our approach and the convergence to the target load distribution.

==> bibliography_MEC.tex <==
%----------------------------------- [1] --------------------------------- 
@article{JAFARNEJADGHOMI201750,
title = {Load-balancing algorithms in cloud computing: A survey},
journal = {J. Netw. Comput. Appl.},
volume = {88},
pages = {50-71},
year = {2017},
issn = {1084-8045},
doi = {https://doi.org/10.1016/j.jnca.2017.04.007},
url = {https://www.sciencedirect.com/science/article/pii/S1084804517301480},
author = {Einollah Jafarnejad {Ghomi} and Amir Masoud {Rahmani} and Nooruldeen Nasih {Qader}},
keywords = {Cloud computing, Load balancing, Task scheduling, Hadoop MapReduce},
abstract = {Cloud computing is a modern paradigm to provide services through the Internet. Load balancing is a key aspect of cloud computing and avoids the situation in which some nodes become overloaded while the others are idle or have little work to do. Load balancing can improve the Quality of Service (QoS) metrics, including response time, cost, throughput, performance and resource utilization. In this paper, we study the literature on the task scheduling and load-balancing algorithms and present a new classification of such algorithms, for example, Hadoop MapReduce load balancing category, Natural Phenomena-based load balancing category, Agent-based load balancing category, General load balancing category, application-oriented category, network-aware category, and workflow specific category. Furthermore, we provide a review in each of these seven categories. Also. We provide insights into the identification of open issues and guidelines for future research.}
}
%------------------------------------- [2] -------------------------------
@article{dsouza2015survey,
  title={A Survey of {Hadoop MapReduce} Scheduling Algorithms},
  author={Dsouza, Mani Bushan},
  journal={Int. J. Innov. Res. Comput. Commun. Eng},
  volume={3},
  number={7},
  year={2015}
}
%-------------------------------------- [3] ------------------------------
@ARTICLE {liu2021game,
author = {C. Liu and K. Li and K. Li},
journal = {IEEE Trans. Cloud Comput.},
title = {A Game Approach to Multi-Servers Load Balancing with Load-Dependent Server Availability Consideration},
year = {2021},
volume = {9},
number = {01},
issn = {2168-7161},
pages = {1-13},
abstract = {In this paper, we focus on request migration strategies among multi-servers for load balancing. Different from the general load balancing problem, we consider it under a distributed, non-cooperative, and competitive environment. Due to the mentioned characteristics, we view our problem from a game theoretic perspective and formulate it into a non-cooperative game among the multiple servers, in which each server is informed with incomplete information of other servers. For each server, we define its expected response time as a disutility function and try to minimize its value. We also take into account server availability, which impacts the processing capacity of a server and thus its disutility. We solve the problem by employing variational inequality (VI) theory and prove that there exists a Nash equilibrium solution set for the formulated game. Then, we propose an iterative proximal algorithm (IPA) to compute a Nash equilibrium solution. The convergence of the IPA algorithm is also analyzed and we find that it converges to a Nash equilibrium. Finally, we conduct some numerical calculations to verify our theoretical analyses. The experimental results show that our proposed IPA algorithm converges to a Nash equilibrium very quickly and significantly decreases the disutilities of all servers by configuring a proper request migration strategy.},
keywords = {servers;load management;cloud computing;time factors;games;nash equilibrium;algorithm design and analysis},
doi = {10.1109/TCC.2018.2790404},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {Jan.}
}
%----------------------------------------- [4] ---------------------------
@article{shi2023,
author = {Shi, Yao and Alsusa, Emad and Baidas, Mohammed W.},
title = {On the Application of Uplink/Downlink Decoupled Access in Heterogeneous Mobile Edge Computing},
year = {2023},
issue_date = {2023},
publisher = {Elsevier North-Holland, Inc.},
address = {USA},
volume = {223},
number = {C},
issn = {1389-1286},
url = {https://doi.org/10.1016/j.comnet.2023.109593},
doi = {10.1016/j.comnet.2023.109593},
journal = {Comput. Netw.},
month = {Mar.}
}
%------------------------------------------ [5] --------------------------
@ARTICLE{Cheng23:DTM,
  author={Cheng, Xiaotong and Maghsudi, Setareh},
  journal={IEEE Trans. Green Commun. and Netw.}, 
  title={Distributed Task Management in Fog Computing: A Socially Concave Bandit Game}, 
  year={2023},
  volume={7},
  number={3},
  pages={1486-1500},
}
%--------------------------------------------- [6] -----------------------
@inproceedings{wang2022decentralized,
  title={Decentralized task offloading in edge computing: A multi-user multi-armed bandit approach},
  author={Wang, Xiong and Ye, Jiancheng and Lui, John CS},
  booktitle={IEEE INFOCOM},
  pages={1199--1208},
  year={2022}
}
%--------------------------------------------- [7] -----------------------
@ARTICLE{Ghoorchian2021,
  author={Ghoorchian, Saeed and Maghsudi, Setareh},
  journal={IEEE Trans. Cogn. Commun. and Netw.}, 
  title={Multi-Armed Bandit for Energy-Efficient and Delay-Sensitive Edge Computing in Dynamic Networks With Uncertainty}, 
  year={2021},
  volume={7},
  number={1},
  pages={279-293},
  doi={10.1109/TCCN.2020.3012445}}
%--------------------------------------------- [8] -----------------------
@book{banez2021mean,
  title={Mean Field Game and Its Applications in Wireless Networks},
  author={Banez, Reginald A and Li, Lixin and Yang, Chungang and Han, Zhu},
  year={2021},
  publisher={Springer}
}
%--------------------------------------------- [9] -----------------------
@inproceedings{gummadi2013mean,
  title={Mean field analysis of multi-armed bandit games},
  author={Gummadi, Ramki and Johari, Ramesh and Schmit, Sven and Yu, Jia Yuan}, 
  booktitle={proc. SSRN},
  year={2013},
  pages={1--28},
  note={[Online]. Available:  \url{https://ssrn.com/abstract=2045842}}  
}
%--------------------------------------------- [10] -----------------------
@ARTICLE{maghsudi2017distributed,
  author={Maghsudi, Setareh and Hossain, Ekram},
  journal={IEEE Access}, 
  title={Distributed User Association in Energy Harvesting Dense Small Cell Networks: A Mean-Field Multi-Armed Bandit Approach}, 
  year={2017},
  volume={5},
  number={},
  pages={3513-3523},
  doi={10.1109/ACCESS.2017.2676166}}
%--------------------------------------------- [11] -----------------------
@inproceedings{mancuso2023efficiency,
  title={Efficiency of distributed selection of edge or cloud servers under latency constraints},
  author={Mancuso, Vincenzo and Badia, Leonardo and Castagno, Paolo and Sereno, Matteo and Marsan, Marco Ajmone},
  booktitle={21st Mediterranean Commun. and Comput. Netw. Conf. (MedComNet)},
  pages={158--166},
  year={2023},
}
%--------------------------------------------- [12] -----------------------
@article{chen2019mobile,
  title={Mobile edge computing based task offloading and resource allocation in {5G} ultra-dense networks},
  author={Chen, Xin and Liu, Zhiyong and Chen, Ying and Li, Zhuo},
  journal={IEEE Access},
  volume={7},
  pages={184172--184182},
  year={2019},
  publisher={IEEE}
}
%--------------------------------------------- [13] -----------------------
@article{guo2022joint,
  title={Joint computation offloading and parallel scheduling to maximize delay-guarantee in cooperative {MEC} systems},
  author={Guo, Mian and Mukherjee, Mithun and Lloret, Jaime and Li, Lei and Guan, Quansheng and Ji, Fei},
  journal={Digit. Commun. and Netw.},
  year={2022},
  publisher={Elsevier}
}
%--------------------------------------------- [14] -----------------------
@ARTICLE{9136780,
  author={Xiao, Liang and Lu, Xiaozhen and Xu, Tangwei and Wan, Xiaoyue and Ji, Wen and Zhang, Yanyong},
  journal={IEEE Trans. Commun.}, 
  title={Reinforcement Learning-Based Mobile Offloading for Edge Computing Against Jamming and Interference}, 
  year={2020},
  volume={68},
  number={10},
  pages={6114-6126},
  keywords={Task analysis;Mobile handsets;Edge computing;Computational modeling;Interference;Energy consumption;Jamming;Mobile offloading;edge computing;interference;jamming;reinforcement learning},
  doi={10.1109/TCOMM.2020.3007742}}
%================================================================================
